A Constant-Factor Approximation Algorithm for Point Guarding an Art Gallery

Given a simple polygon $\cal P$, in the Art Gallery problem the goal is to find the minimum number of guards needed to cover the entire $\cal P$, where a guard is a point and can see another point $q$ when $\overline{pq}$ does not cross the edges of $\cal P$. This paper studies a variant of the Art Gallery problem in which guards are restricted to lie on a dense grid inside $\cal P$. In the general problem, guards can be anywhere inside or on the boundary of $\cal P$. The general problem is called the \emph{point} guarding problem. It was proved that the point guarding problem is APX-complete, meaning that we cannot do better than a constant-factor approximation algorithm unless $P = NP$. A huge amount of research is committed to the studies of combinatorial and algorithmic aspects of this problem, and as of this time, we could not find a constant factor approximation for simple polygons. The last best-known approximation factor for point guarding a simple polygon was $\mathcal{O}(\log (|OPT|))$ introduced by E. Bonnet and T. Miltzow in 2020, where $|OPT|$ is the size of the optimal solution. Here, we propose an algorithm with a constant approximation factor for the point guarding problem where the location of guards is restricted to a grid. The running time of the proposed algorithm depends on the number of cells of the grid. The approximation factor is constant regardless of the grid we use, the running time could be super-polynomial if the grid size becomes exponential.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file

